Multimodal Transformer Distillation for Audio-Visual Synchronization

Audio-visual synchronization aims to determine whether the mouth movements and speech in the video are synchronized. VocaLiST reaches state-of-the-art performance by incorporating multimodal Transformers to model audio-visual interact information. However, it requires high computing resources, making it impractical for real-world applications. This paper proposed an MTDVocaLiST model, which is trained by our proposed multimodal Transformer distillation (MTD) loss. MTD loss enables MTDVocaLiST model to deeply mimic the cross-attention distribution and value-relation in the Transformer of VocaLiST. Additionally, we harness uncertainty weighting to fully exploit the interaction information across all layers. Our proposed method is effective in two aspects: From the distillation method perspective, MTD loss outperforms other strong distillation baselines. From the distilled model's performance perspective: 1) MTDVocaLiST outperforms similar-size SOTA models, SyncNet, and Perfect Match models by 15.65% and 3.35%; 2) MTDVocaLiST reduces the model size of VocaLiST by 83.52%, yet still maintaining similar performance.

==> content/4.experiment/table/abla_differ_weight_tab.tex <==
% Ablation Study of the embedding loss of AVADL new
\begin{table}[t]
% \renewcommand{\tabcolsep}{3.8pt}
% \renewcommand{\tabcolsep}{4.2pt}
% \renewcommand{\tabcolsep}{3.0pt}
\renewcommand{\tabcolsep}{3.5pt}
\renewcommand\arraystretch{1.2}
\small
% \fontsize{8}{10}\selectfont
% \fontsize{9}{10}\selectfont
% \fontsize{9}{9}\selectfont
\vspace*{-0.4cm}
\caption{Accuracy for models trained with different weights.}
\centerline{
\begin{tabular}{c|c|c|c|c|c|c}
\hline
\multirow{3}{*}{\shortstack[c]{Weighted \\
method}} & \multicolumn{6}{c}{Input frame length (seconds)} \\
\cline{2-7}
% \hline
           &  \multirow{2}{*}{\shortstack[c]{5 \\ (0.2s)}}  &  \multirow{2}{*}{\shortstack[c]{7 \\ (0.28s)}}    &    \multirow{2}{*}{\shortstack[c]{9 \\ (0.36s)}}    &  \multirow{2}{*}{\shortstack[c]{11 \\ (0.44s)}}      & \multirow{2}{*}{\shortstack[c]{13 \\ (0.52s)}}      & \multirow{2}{*}{\shortstack[c]{15 \\ (0.6s)}} \\
           &       &   &   &   &  &  \\

\hline
\hline
 Uniform  &   91.08   &   95.56   &    97.77   &   98.82   &  99.39    &   99.67   \\
\hline
AW-13D    &   \textbf{91.23}   &   \textbf{95.68}   &  \textbf{97.94}  &   \textbf{98.96}   &  \textbf{99.48}    &   \textbf{99.71}   \\
AW-25D    &   91.02     &   95.60   &   97.76   &   98.87    &   99.41   &  99.69   \\

\hline

\end{tabular}}
% \vspace*{-0.3cm}

% \vspace*{-0.3cm}
\label{tab:acc_of_diff_weight}
\end{table}

